Application Performance Modeling via Tensor Completion

Performance tuning, software/hardware co-design, and job scheduling are among the many tasks that rely on models to predict application performance. We propose and evaluate low-rank tensor decomposition for modeling application performance. We discretize the input and configuration domains of an application using regular grids. Application execution times mapped within grid-cells are averaged and represented by tensor elements. We show that low-rank canonical-polyadic (CP) tensor decomposition is effective in approximating these tensors. We further show that this decomposition enables accurate extrapolation of unobserved regions of an application's parameter space. We then employ tensor completion to optimize a CP decomposition given a sparse set of observed execution times. We consider alternative piecewise/grid-based models and supervised learning models for six applications and demonstrate that CP decomposition optimized using tensor completion offers higher prediction accuracy and memory-efficiency for high-dimensional performance modeling.

==> application_notes.tex <==
General observations
GEQRF
- no improvement beyond rank 4/5. Rank-3 is already very good. Quite easy kernel to model.


ExaFMM
- a higher order of expansion (P) uses more memory.
- higher number of bodies per leaf (ncrit) uses less memory for a fixed order of expansion.
- numBodies is specified per process. Therefore, I want to make sure that only between 4096 and 65536 bodies exist per node.
- m2l_&_p2p is the kernel we test (not total_fmm)

AMG
- 3D Laplacian for convection/diffusion, {solver type, smoother type, interpolator type, coarsening type, elements/row, core/uncore frequency, hyperthreading switch}
- Confirmed that the smaller PPN count datasets are easier to model, thus making the 8D dataset easier to model than the 6D with ppn=64.
- There is a huge difference between log-transformed data and non-log-transformed data (unlike with ExaFMM)
- For a fixed (node,ppn,tpr)==(1,64,1):
  Min time - 0.276308
  Max time - 391.907783
  
Uncertain things:
1. nx,ny,nz is per process (I think this is the right way to model weak scaling).
2. Perhaps not enough samples for a test set
3. Have not tested extrapolation yet
4. Missing node counts 64,128,256,512

Full tensor should be ZxZxZx7x10x14x7x7x6
No modes for P,Q,R (processor grid shape) as they are strongly correlated with process count.


==> autotuning_text.tex <==
  \subsection{General-purpose autotuners}
    General-purpose autotuners must provide efficient mechanisms for configuration space generation, storage, and search.
    Recently, the presence of interdependencies among tuning parameters has proven critical influence of each phase.
    Orio\cite{hartono2009annotation}, OpenTuner\cite{ansel2014opentuner}, and libtuning\cite{pfaffe2019efficient} keep invalid configurations within search space and thus inhibit the efficiency of the three phases, including search.
    As OpenTuner and libtuning consider all configurations valid, they need not consider efficient generation and storage of search space.
    Configurations can be generated on-the-fly as combinations of individual parameter values.
    Standard search methods work well on such a representation, because each subspace is mapped to a coordinate space (collection of equally-spaced real numbers), upon which numerical search techniques are made for.
    Explicitly-provided penalty value for invalid configurations to suffice.
    ATF notices that well over 99 percent of configurations can be invalid, precluding such frameworks from being efficient.
    KernelTuner, ActiveHarmony\cite{tiwari2009tuning}, and CLTune\cite{nugteren2015cltune} take into account these interdependencies, but are not as efficient as they could be (see below).
    They only care about the effect on the search method, and store each valid configuration explicitly, thus running up memory footprint and increasing generation time and storage cost.
    These frameworks operate on a constrained search space, write all valid configurations to a 1D array, and use search methods that operate on that 1D array.
    ATF\cite{rasch2021efficient} proposes a chain-of-trees mechanism to efficiently generate, store, and search configuration spaces defined by tuning parameters that have interdependencies among them.
    ATF leverages a different constraint specification than CLTune and KernelTuner\cite{van2019kernel}.
    ATF however does not construct a surrogate model, and thus has no support for multi-task autotuning.
    ATF builds constraints locally, with individual parameters referencing previously defined parameters, while the other two take a whole configuration and use members of the configuration to decide whether or not the configuration is legal.
    ATF relies on parameter constraints, CLTune and KernelTuner rely on configuration space constraints, OpenTuner allows no constraints.
    ATF allows simple specification of user parameters: just specify the name, range, and constraints.
    As such, CLTune and KernelTuner generate seach spaces by iterating over deep nested loops over the ranges of each parameter, and use the lambda within that.
    So constraints must be checked at the deepest nested loop level, allowing no chance to prune, which constraints specified at the parameter level do.
    ATF on the other hand, can leave early, by checking a parameter's locally-defined constraints at every loop-nest level.
    Further, ATF's parameter-based constraints allow for simple partitioning into groups of interdependent tuning parameters.
    Exploiting this makes the generation of the search space faster, as each group can be handled in parallel.
    Within each group, the generation of the search space can be handled in parallel.
    CLTune and KernelTuner's constraint specification design precludes automatic identification of such groups.
    Another form of parallelism in search space generation beyond handling each group independently: parallel-for over the outer-most loop corresponding to the parameter with no constraints (ATF uses a thread-pool to manage this and avoid parallelism overhead). 
    Two parameters are considered interdepent if one exists in the syntax tree (via constraint) of the other
    Realize that a group of interdependent tuning parameters is identified by constraint only, not by influence on execution time.
    Thus, each tuning parameter group cannot be tuned independently (see BLISS for a nice illustration of the downsides of doing this).
    Our approach does not need to take into account constraints when building the configuration space, only when specifying the next set of configurations surrounding well-performing ones to next sample as part of the next batch.
    {\color{red}I think our approach avoids all of this funny business by representing the space as a low-rank tensor}.
    With the exception of GPTune, none of these libraries has efficient mechanisms for multi-task learning.
    \par
    {\color{red}How does GPTune's infrastructure compare?}
    Halide paper with new parameterization and search method.
    
    
  Autotuning has been the subject of considerable and varied research.
  {\color{blue}We do not want to compete against special-purpose autotuners.}
  We believe our approach is the first scalable approach towards multi-task autotuning, that leverages a new assumption.
  Our approach factors into account the execution times themselves in determining the storage space of the multi-task configuration space.
  Our approach can also be systematically improved using higher rank.
  We demonstrate that generation and storage of search spaces is not a huge problem if individual modes are contrained together as we do.
  \par
  
  \section{Configuration Space Representation using Matrix Rank}

  The accuracy and scalability of performance modeling frameworks and autotuning search techniques in predicting application performance is highly sensitive to the representation of the application's configuration space {\color{red}(cite ATF,SGR)}.
  Model-free search techniques enumerate each parameter's value range along a distinct mode of an $N$-dimensional tensor {\color{red}(cite)}, a lightweight representation optimal for optimizing an objective across an unconstrained (i.e., every combination of parameters is feasible) $N$-dimensional configuration space {\color{red}(cite)}.
%  While such a representation is storage and time efficient, it is not appripriate when the ...
  The presence of parameter constraints segments a configuration space into feasible and infeasible subspaces.
  Studies have shown that this can significantly inhibit search techniques designed for tensor configuration space representations {\color{red}(cite)}.
  Alternative representations enumerate all feasible $N$-parameter configurations along a single tensor fiber (i.e., 1D array) {\color{red}(cite)} or classify tuning parameters by constraint into parameter groups in a chain-of-trees representation{\color{red}(cite)}.
  Search efficiency priorized by these techniques preclude learning the interactions among tuning parameters necessary for accelerated autotuning across tasks and machines.
  \par

  The predominant approaches to online model construction during autotuning leverage Bayesian optimization.
  Gaussian processes (i.e., multi-dimensional Gaussian distributions) act as surrogate models for the .
  In short, every possible configuration has a prediction, but comes with uncertainty.
  Large covariance matrix effectively serves as the representation, and grows with ....
  Various efforts have been designed to allow this.
  Surrogate models are constructed online during tuning. for , which have been extended to allow multi-task learning.
  Here, discuss models for entire configuration space.
  In contrast, surrogate models aim ..that leverage Gaussian processes incur solves, but ... Surrogate models using the linear coregionalization method have been shown to . Ultimately, these methods are limited by the size of the search space, and rely on a variety of surrogate kernels {\color{red}(cite)}.
  \par

\subsection{Metrics}

  The work performed by a kernel $K$ is characterized by $M$ task parameters $t_{1},...,t_{M}$. The execution time $T$ to complete a task's work is influenced by $N$ tuning parameters $p_{1},...,p_{N}$. As such, $T_{K_{(\tilde{t}_{1},...,\tilde{t}_{M})}}(\tilde{p}_{1},...,\tilde{p}_{N})$ represents the execution time of a particular configuration $(\tilde{p}_{1},...,\tilde{p}_{N})$ of task $K_{(\tilde{t}_{1},...,\tilde{t}_{M})}$. For example, $T_{GEMM_{(10^{2},10^{4},10^{1})}}(64,16,8)$ represents the execution time of multiplying $C=A_{10^{2}\times 10^{4}}B_{10^{4}\times 10^{1}}$ using $64$ threads and square cache and register tiles of dimensions $16$ and $8$, respectively. As we propose to represent a kernel's execution time across its parameter space $T_{K_{(t_{1},...,t_{M})}}(p_{1},...,p_{N})$ as a low-rank $M+K$-dimensional tensor, we are first interested in establishing metrics that measure interactions among tuning parameters.
  \par

  The execution times measured when varying the values assigned to a pair of tuning parameters $p_{i},p_{j}$ for a particular task can be represented by a matrix $A_{i,j}$, assuming the remaining $N-2$ tuning parameters are held constant.
  The singular value decomposition (SVD) of $A_{i,j}$ offers insight into whether parameters $p_{i},p_{j}$ should be characterized together along the same mode and within the same group.
  In particular, we are concerned with the number of singular values $\sigma$ necessary to achieve a low-rank representation $U\Sigma V^{T}$.
  The ranges of two tuning parameters $p_{i},p_{j}$, if the rank of the execution times of all value pairs is low, our model benefits from keeping these parameters along separate modes. However, if the rank is high, our model should not assume presence of low-rank and thus keep them along the same mode. Without careful ..., such a prediction can be compromised. For example, if $K$ is too large (say $K=M+N$), the model may assume the presence of low-rank interactions among task and tuning parameters when they don't exist. However, if $K$ is too small (say $K=M+1$) and thus all tuning parameter configurations for each task are laid out in a 1D array (similar to KernelTuner and others, cite here), which, for our model specifically, would create a very sparse tensor that would inhibit prediction.
  The decisions as to which tuning parameters to group together are determined by balancing trade-offs between tensor sparsity and tensor rank.
  Our model benefits from keeping tuning parameters with little interaction along the same mode, and thus within the same parameter group {\color{red}(need to define group)}.
  Tuning parameters whose varied values produce execution times with low-parameter interaction belong on separate modes so that our model can leverage itself.
  {\color{red}Discuss groups of tuning parameters.}
  \par

  We propose to represent a kernel's parameter space that leverages the rank of the interactions among groups of tuning parameters. We first propose a methodology and then refine it to make it efficient.
  \par

  {\color{red}Question: can other performance prediction methods leverage this parameter-space representation?}
  \par

  {\color{red}Need to define the tuning parameters, tuning parameter groups, and the graphical structure that encapsulates this, $G$. Also, need to define the how the assumptions, including the usage of random variables and the distributions being governed by the individual distributions of each tuning parameter (i.e., the value range each can take on, as specied externally).}
  We denote each tuning parameter as a disjoint set. Our goal is to incrementally identify groups od tuning parameters that should not interact due to full rank.
  \par

  Tuning parameters are sampled, while task parameters are more or less discretized in the methodology below.
  \par

  Treat as sampling problem. The sample space is the concatenation of all the task parameters, and the remaining $N-2$ tuning parameters. The distribution of this space is determined by that of the distribution of all parameters. Thus, a sample will simply be a choice of $T+N-2$ parameters. For each sample, we execute all values of each pair of tuning parameters, and perform a SVD on the resulting matrix to attain all singular values. These singular values will give information of how well-approximable the matrix is by a low-rank approximation. The rank necessary to achieve a certain weight is cast as a random value. We are interested in the corresponding sample mean. We start with a number of disjoint sets, each representing a mode of the low-rank tensor representation of the parameter space. At the end, we have a tensor mode for each connected component.
  \par

\subsection{Methodology for Group Construction}

  \begin{algorithm}
  \caption{Parameter Space Construction}\label{alg:v1}
  \KwData{$G: \{\{t_{0}\},...,\{t_{n}\}\}$}
  \KwData{$\epsilon$: Frobenius norm error tolerance}
  \KwData{$\delta$: confidence interval wifth for sample mean of smallest matrix rank that achieves $\epsilon$}
  \KwData{$k_min$: minimum number of full-matrix samples for each TPG pair}
  \KwData{$N_{min}$: minimum number of TPGs}
  \KwResult{$G$}
  $max\_frob_error\gets \infty$\;
  \While{$|G|>N_{min}$ or $max_frob_error>\epsilon$}{
  \Comment*[r]{Initialize sample-mean ranks for all pairs}
  $R\gets 0_{m\times n}$\;
  \For{$i=1\rightarrow|G|$}{
    \For{$j=i+1\rightarrow|G|$}{
      $\tilde{k}\gets 0$\;
      $\tilde{\delta}\gets\infty$\;
      \Comment*[r]{Compute full matrix slices for every pair of TPGs via sampling}
      \While{$k<k_{min}$ or $\tilde{\delta}>\delta$}{
        $A\gets 0_{|G_{i}|\times|G_{j}|}$\;
        $S\gets Sample(...)$\;
        \For{$\hat{i}=1\rightarrow|G_{i}|$}{
          \For{$\hat{j}=1\rightarrow|G_{j}|$}{
            $A_{i,j}\gets Execute(S,\hat{i},\hat{j}$\;
          }
        }
        $\vec{\sigma}\gets SVD(A)$\;
        $\hat{k},\tilde{\epsilon}\gets argmin_{\hat{k}}\frac{||\vec{\sigma}_{\hat{k}}||}{||\vec{\sigma}||}$ s.t. $\frac{||\vec{\sigma}_{\hat{k}}||}{||\vec{\sigma}||}\leq\epsilon$\;
        $R_{i,j} \gets R_{i,j}+\frac{\tilde{\epsilon}}{\hat{k}}$\;
        \Comment*[r]{Update standard error and CL length $\tilde{\delta}$}
        $k\gets k+1$\;
      }
    }
  }
  $(i,j)\gets argmin(R,some metric)$\;
  $G.merge(i,j)$\;
  $max_frob_error\gets ...$\;
  \Comment*[r]{When we get here, we are confident in the sample means in $R$}
  \Comment*[r]{At this point, the tuning parameter group structure has been updated and we can recurse}
  }
  \end{algorithm}

  This methodology should work. However, there are concerns:
  \begin{enumerate}
    \item {\color{red}The parameter range for a particular tuning parameter $t_{i}$ may be excessively large, making the matrices $A_{i,*}$ very large. This would induce excessive execution time, as well as more expensive SVDs.} {\color{green}We could discretize or sample with some distribution} {\color{blue}Possible ablation study: show limiting returns from larger sample sets and finer discretizations.}
    \item {\color{red}A SVD is necessary to get the random variable value for each inner-loop iteration.} {\color{green}I am working on a few proofs here that might avoid this.}
    \item {\color{red}Matrices $A$ might be sparse due to parameter constraints.}{\color{green}Matrix completion is not approrpriate because the matrix may be high-rank. Further, a fixed rank should not be imposed, as that defeats the purpose of what this algorithm is aiming to achieve. However, note that the presence o constraints does not deter our tensor completion performance model, so there is no reason to penalize constraints among tuning parameter pairs and thus force a merge solely because of this. My current solution is to place a zero at each entry in $A$ that violates a constraint.}
    \item {\color{red}By merging two parameter groups, the mode length corresponding to the updated parameter group will increase multiplicatively, creating larger matrices $A$.} {\color{green}For similar reasons as above, folding into a tensor and performing tensor completion is not appropriate. I already tried performing all merges at once, but it resulted in tensors that were too large. Another option is to find the TP group with the smallest $\tilde{\epsilon}/\hat{k}$, merge it, and do the same with all other tuning parameter groups excluding the two just merged. This would result in at most 2x less modes per outer iteration.}
    \item {\color{red}By adding just a single edge at a time, we incur significantly increased sample time, as we need to re-sample for every update to $G$.} {\color{green} We could re-discretize to keep the matrix dimensions under control.}
    \item {\color{red}No clear way to incorporate the number of values a tuning parameter can take into the merging decisions beyond dividing $\tilde{\epsilon}$ furhter by it.}
    \item {\color{red}Should the training set for determining the factor matrices be separate from the samples attained via this approach?}
    \item {\color{red}What transformation of the data to use before calling SVD?}
  \end{enumerate}

  After each simulation, each pair of tuning parameters has associated with it an SVD. If tuning parameter pair $(i,j)$ should be merged, this means that for any $k$ s.t. $A_{i,k}$ and $A_{j,k}$ previously existed, with ranks $r_{i,k}$ and $r_{j,k}$, respectively, they must get merged into a single matrix $B_{(i,j),k}$. The point of merging is to avoid any assumption of low-rank between them for our TC model.
  \par
  Understand that with matrix $B_{(i,j),k}$, the random variable underlying the sampling has changed: one less outside parameter is being selected, or equivalently two are being fixed rather than one. The problem with using a RV or the execution time of every element of a slice was that the choice of all other variables can have a signiicant impact, thus preventing any stabilization of the distribution. The sample mean would be all over the place.
  \par
  The singular values attained for each slice are needed to determine which rank achieves a Frobenius norm ratio of $\epsilon$. We treat the measure $\epsilon/\hat{k}$ as a random variable, and are interested in its sample mean, which means we need to call a SVD for each slice. There exist a number of interesting inequalities, including $\Sigma_{i=1}^{n}\sigma_{i}(A+B)\leq \Sigma_{i=1}^{n}\sigma_{i}(A)+\Sigma_{i=1}^{n}\sigma_{i}(B)$. {\color{blue}Understand that the whole point of this is that I want to focus at the granularity of the single matrix $\Sigma_{i=1}^{k}A_{j}$, but I need to understand how that compares to dealing with each matrix $A_{j}$ separately as described in the above methodology.}
  \par
  Something we know: $\Sigma_{i=1}^{N}[\Sigma_{j=\hat{k}_{i}}^{n}\sigma_{j}(A_{i}) / \Sigma_{j=1}^{n}\sigma_{j}(A_{i})] \leq N\epsilon$. We need to show that this is achievable using a sum of matrices, perhaps with the caveat that we drop the per-sample requirement that for each slice $i$ $\tilde{\epsilon}<\epsilon$ (which we wouldn't know anyways). Could perhaps call this aggregation-weight based, rather than per-sample based. If we used this, we'd need to prove that the sum-of-matrix approach hits an upper bound of $\Sigma_{i=1}^{N}[\Sigma_{j=\hat{k}_{i}}^{n}\sigma_{j}(A_{i}) / \Sigma_{j=1}^{n}\sigma_{j}(A_{i})]$. Using a proof, we know $\Sigma_{i=1}^{n}\sigma_{i}(\Sigma_{j=1}^{N}A_{j}) \leq \Sigma_{i=1}^{n}\Sigma_{j=1}^{N}\sigma_{i}(A_{j})$, which means that $\frac{\Sigma_{i=k}^{n}\sigma_{i}(\Sigma_{j=1}^{N}A_{j}}{\Sigma_{i=1}^{n}\sigma_{i}(\Sigma_{j=1}^{N}A_{j})}\leq\frac{\Sigma_{i=k}^{n}\sigma_{i}(\Sigma_{j=1}^{N}(A_{j})}{\Sigma_{i=1}^{n}\Sigma_{j=1}^{N}\sigma_{i}(A_{j})}$. {\color{red}But aren't I going the wrong way here with that initial inequality? In my notes, I have that I'd then need to show that $\Sigma_{i=k}^{n}\sigma_{i}(\Sigma_{j=1}^{N}A_{j})\leq\Sigma_{j=1}^{N}\Sigma_{i=\hat{k}_{j}}^{n}\sigma_{i}(A_{j})$, but I need to verify that math.}
  \par

  From Terrance Tao's provided Lidskii Inequality, it's quite clear that there is no guarantee that the sum of the first $k$ singular values of $A+B$ will yield as big of mass as the separate sum of singular values. This inequality also didn't provide a way to use different $\hat{k}_{i}$ for each slice $i$. Leveragint the fact that all matrices are positive does not change anything.\par

  Two inequalities have been confirmed experimentally. The first is known, while the second might not be:
  \begin{enumerate}
    \item $\Sigma_{i=1}^{k}\sigma_{i}(\Sigma_{j=1}^{N}A_{j})\leq \Sigma_{j=1}^{N}\Sigma_{i=1}^{k}\sigma_{i}(A_{j})$
    \item For all $1\leq k\leq min(m,n)$, $\frac{\Sigma_{i=1}^{k}\sigma_{i}(\Sigma_{j=1}^{N}A_{j}}{\Sigma_{i=1}^{n}\sigma_{i}(\Sigma_{j=1}^{N}A_{j})}\leq 1/N[\Sigma_{j=1}^{N}[\frac{\Sigma_{i=1}^{k}\sigma_{i}(A_{j})}{\Sigma_{i=1}^{n}\sigma_{i}(A_{j})}]]$
  \end{enumerate}
  The second inequality I'd have to prove formally, but I would also need to prove an additional statement that guarantees that using the sum-of-matrix measure, the most high-arank tuning parameter pair is always chosen. This second inequality means that if I operate with the sum of slices, and I detect that rank $\tilde{k}$ achieves $(1-\epsilon)\%$ of the mass according to the Frobenius norm, that covers at least as much as the arithmetic mean of each slice at the same rank covers individually, which is slightly weaker than our methodology, which treated the detected rank individually.
  \par

  I also confirmed experimentally that the following does not hold when trying to prove the above: for any $1\leq i\leq n$, $\frac{\sigma_{i}(\Sigma_{j=1}^{N}A_{j}}{\Sigma_{k=1}^{n}\sigma_{k}(\Sigma_{j=1}^{N}A_{j}}\geq 1/N\Sigma_{j=1}^{N}[\frac{\sigma_{i}(A_{j})}{\Sigma_{k=1}^{n}\sigma_{k}(A_{j})}]$.

  Note that a problem with my attempts above is that they rely solely on the Frobenius norm ratio of singular values, when I know from the specified tolerance $\epsilon$ that all will achieve the necessary amount. The interesting thing is with which percentage of its singular values is it achieved. Therefore, we need to utilize the rank in some way, although if we prove an inequality or any streak of singular values, that may suffice. Another problem is that if we operate with a sum of matrices, how can we know when to stop executing new slices, given that we no longer have access to the singular values per slice if we don't want to call an SVD per-slice? One idea that we shouldn't adopt is to instead have the user specify a tolerance based on the rank itself, rather than the Frobenius norm mass. An idea that may have merit is to utilize per-element-of-slice random variables that act as a fraction of the execution times across the entire slice, which may stabilize.
  \par

  If we define $\bar{\epsilon}=\tilde{\epsilon}\cdot min(m,n)/rank$, we need to show that using a sum of slices, $\bar{\epsilon}_{i,j}>\bar{\epsilon}_{i^{'},j^{'}}$ iff $AM[\bar{\epsilon}_{i,j}]>AM[\bar{\epsilon}_{i^{'},j^{'}}]$. We can drop out $\tilde{\epsilon}$ from the expression, as it will always be bounded from above by $\epsilon$. I would hope we could use the ideas expressed above to prove such a thing, but again, still need to find some way to stop sampling.
  \par

  We still want to use a disjoint set, just use it incrementally.
  \par

  To summarize, we need to prove two ideas in order to justifiably operate at the coarser granularity of sums of slices, and thus avoid calling a SVD for each slice:
  \begin{enumerate}
    \item There exists a way to know when to stop executing slies that is near-equivalent to using $\delta$ with the above methodology.
    \item Need to show that for contracted slices, $\bar{\epsilon}_{i,j}>\bar{\epsilon}_{i^{'},j^{'}}$ iff AM$[\bar{\epsilon}_{i,j}]>$AM$[\bar{\epsilon}_{i^{'},j^{'}}]$.
  \end{enumerate}
  In short, we must account for $\delta$ and $\epsilon$ in the above methodology. {\color{red}We also need to show that it is justified to drop the per-slice requirement of achieving $\tilde{\epsilon}<\epsilon$ and that achieving it for matrix of contracted slices is sufficient.}
  \par

  {\color{red}The execution time needed to fill a slice should dwarf that of performing a SVD, making some optimizations un-needed for now}. Another optimization is to carefully choose task parameters so that they are small, while still being sufficiently representative. Linearlly-spaced on a logarithmic scale should be appropriate.
  \par
  
  
  These published analytical models are used as an argument against empirical search, which can be wasteful, especially across many different problem sizes, and also do not allow for analytical insight (although recent approaches are handling multi-task autotuning, etc.).
  
  \textit{Demand for autotuning has been identified as a major research challenge in high-performance computing}\cite{balaprakash2018autotuning,basu2013towards}
  
  A kernel's performance is often sensitive to the setting of hardware and tuning parameters, which motivates single-task autotuning.
  The difficulty of predicting a kernel's performance given a selection of parameters is exacerbated when considering many distinct tasks, hence the recently proposed techniques for multi-task autotuning\cite{liu2021gptune}.
  We evaluated the scalability of this technique and found that the number of model parameters necessary to accurately predict kernel performance across many parameters can be exorbitant, precluding its use as an accurate surrogate model for a number of kernels.
  Gaussian processes\cite{liu2021gptune} and deep neural networks\cite{lee2007methods} offer alternative approaches to predicting kernel performance.
  However, the scalability of Gaussian process regression is hindered by the necessity of storing and inverting covariance matrices, while deep neural networks must be trained with sufficiently large training sets, are difficult to interpret, and offer limited opportunities to attain tunable, user-customized prediction accuracy.
  \par
  
  End-to-end deep learning of optimization heuristics - one of the first to propose a tool that does not require expert knowledge to construct features.
  
  Algorithms designed to attain the performance available on this increasingly large set of architectures are in turn becoming increasingly complex.
  State-of-the-art performance models seek to accurately predict the execution time of many distinct tasks, yet are ill-suited to modeling task configuration spaces without offline statistical analysis {\color{red}(cite)}.
  State-of-the-art search techniques (e.g., simulated annealing, genetic algorithms, multi-armed bandit) seek the optimal $N$-parameter configuration for a particular task, yet avoid constructing a surrogate performance model and thus cannot learn the interactions among tuning parameters across tasks.
  1. Task parameters: describe the problem to be solved (amount of Work).
  2. Hardware parameters: describe the hardware with which to solve the problem (the resources with which to complete the work, determines the Time, think work-time model)
  3. Tuning parameters: describe application-level tuning knobs that can vary the cost (e.g., synchronization, communication, computation) and thus the resulting execution time.
  
  Our model's insensitivity to offline statistical analysis and critical-path analysis seems particularly attractive as a surrogate model for autotuning.
  Leave off more general generalized CP-ALS using distribution-aware.
  Generate models within cells to optimize for better error at lower sample count (less reliance on distance alone).
  Don’t restrict training set to grid-points only (use quadarature within cell).
  Identify whether the right Bayesian surrogate model across a configuration space (BLISS studies single-task).
  
    Compilers predominantly rely on imprecise cost models for selecting tile-sizes and loop-permutations, among other important tasks.
    Program optimization, enabled by online tuning parameter selection, often is delayed until input characteristics, including sparsity and .., only available at execution time.
    
    Compilers predominantly rely on imprecise cost models for selecting tile-sizes and loop-permutations, among other important tasks.
    Program optimization, enabled by online tuning parameter selection, often is delayed until input characteristics, including sparsity and .., only available at execution time.
    
    
    Nonlinear approximation to statistical relationships among inputs.
    These methods utilize bootstrapping to train multiple trees.
    A random subset of features is chosen to formulate decisions at each node, and the best split is chosen per some metric.
    Original work:~\cite{breiman2001random}.
    Related works on algorithm prediction via generation of ML surrogate models ~\cite{hutter2011sequential,baz2007automated,bartz2004tuning,marathe2017performance,wu2020autotuning,sun2020automated}.\\

==> extrapolation.tex <==
Formalize extrapolation problem statement. Goal is to provide robust predictions to inputs outside of the modeling domain. How we define this is subject to interpretation but we must provide examples, especially from autotuning. The question of when to interpolate, extrapolate, or execute a given input must be defined clearly and is related to this item.

Extrapolation environment 1: at least one input within d-parameter configuration is outside of the modeling domain ascertained during training from the training set. In this case, we currently default to use of a rank-1 factorization. This will showcase model accuracy with decreasing information (as the diagram showcases). Keep size of training set fixed as well, so randomly sample from the procured training set. Keep test set fixed as large as possible within the larger range.

Extrapolation environment 2: all inputs within d-parameter configuration are inside the modeling domain ascertained during training from the training set, yet the sampling region is zero within the corresponding cell. This is more subtle because such a situation may arise often if the density is spread out. This may be more indicative of high-dimensional extrapolation than the previous environment. This bleeds into modeling with parameter constraints, for which we'll need to think of distinct experiments. The key question here is is there any benefit with higher rank in this extrapolation regime?

Re-plot the factor matrices with this new scaling constant, starting with CP rank 1, with a baseline range (x-axis being the range, not the indices since we can always just place 32 grid-points as long as the training set is large enough). We can then picture how accurate the extrapolation scheme is or can be as we vary CP rank. Include the contracted tensor data t_ijk / (v_1,j*w_1,k) to see how well the factor matrix column data fits it.


BELOW is old.

Realize that as we are extrapolating across problem sizes for GEMM, there are hidden tuning parameter selection under the hood dependent on problem size. Thus, if these change across the cut, there is no expectation to model them correctly.


Question: if we are ultimately performing regression anyways with tensor completion, must our model pass through all of the factor matrix elements? Yes in the linear interpolation case, but that is not necessarily the best approach. SGR is stuck with linear regression with many grid-points, but this may help us with smaller training sets?



1. Our current extrapolation scheme is most robust when there is sufficiently many rows of each numerical (i.e., non-categorical) application benchmark parameter. However, one cannot simply increase the number of rows without a sufficiently large training set, else the factor matrix elements will not be amenable to linear regression.
- This is currently a problem for architectural parameters, for which it is expected to have few rows of the corresponding factor matrix.


In general:
From the factor matrix data, we see that as rank increases, there is more variation in the factor matrix data. This is problematic for extrapolation specific to this method, so see if, by changing the regularization, we can mitigate this variation. So for this to work, we need sufficiently high regularization.

The extremes are the current model with a grid-point placed and linear models in each gap, and the other extreme is a curve through all factor matrix elements. For extrapolation, we'd like the latter option to be best. If the data is too jagged, then extrapolation will not be accurate. Regularization may help to avoid jagged-ness, but is not sufficient. The free parameters in this scheme are where to place grid-points (none to all) and which degrees to try between grid-points (line to max-spline-degree specified by user). MARS does both automatically but is too heavy-handed. We want to give the full curve every opportunity to exist, and we will start from one extreme (all grid-points and linear models between each pair). While this is perfect for interpolation, it is not right (linear extrapolation) for extrapolation. We'd like to penalize the initial setup unless the fit is just too good. Initially, the GCV will literally be 0 because the model will perfectly predict the factor matrix data. We need to figure out a way to circumvent this. We really only need a backward pass if we compare to MARS, as we will start with the most complex model possible for each factor matrix column. The fact that the initial RSS is 0 is kind of meaningless, yet we can never improve upon it, which is a challenge. Further, we do want to keep at least a few of the grid-points in the extrapolation model, which will contribute 0 to RSS as well. We should thus start instead with a forward pass and not bother with a backward pass. Start with no grid-points, then search over the placement of 1 grid-point at the specified locations, and try from 0 up to max-spline-degree. Then, we can see if we can move forward towards the placement of 2 grid-points in a greedy fashion (so fix the first one found in the previous step). Greedy, not backtracking.

Larger region for extrapolation (e.g., cut 512): linear least-squares with a global model fit to each FM column is far superior to linear extrapolation.
Small region for extrapolation (e.g., cut 2048): linear extrapolation using two closest is superior.
Mention that we utilize this linear extrapolation currently to model stuff in the paper outside of the end mid-points.
We don't need any extra memory to perform linear extrapolation.

Extrapolation should act as a switch: close enough to the training data region of a particular mode? use linear extrapolation. Too far away? use a simple global model.

Idea: we want the linear fit to be weighted towards the end-points, so we can simply leverages the typically bad properties of LLS before transformation of data to get the fit to be better with data closer to larger ends of region. This may largely alleviate the need to use a MARS-like procedure, since we wouldn't use these models for interpolation within the training region anyways.
However, this may not be possible due to the log-transformation we already take prior to optimizing the FM elements, and we may instead want to work from the end-points n both sides and work our way until the fit is best. A size-2 would always have a RSS of zero, so we must limit the smallest window to 3 FM elements. We could also add an additional penalty that is high for small numbers of points.
I observe that the residual when fitting 3 points is often far less than that of fitting N points. However, fitting 3 points is still superior to linear extrapolation, so if 3 points yields a good fit, we should trust it.

Extrapolation just isn't truly needed within an interpolation region, even if there is a large gap. However, we can think about it in a MARS-like fashion later if necessary. We already know that log-spacing is almost always superior to other spacings.

Note that I started with this because it was easiest to place an extra grid-point that encloses all possible entries (this isn’t necessarily practical since we may not know what the end-point is) without any other changes to code. Keep this file though.



Scratch work on CPR extrapolation

Observations and conclusions:
- Variation is not specific to a single factor matrix (following normalization), which is healthy. This can sometimes be difficult to notice, but if we normalize to avoid negatives and plot on log-scale, it is clear.
- Piecewise-linear behavior is concerning for extrapolation, as such behavior cannot be easily extrapolated from small-input data. Excess regularization could help here.
- We are fine with generating lots of small data, so extrapolation is really more important for larger problem sizes. No reason not to execute a tiny GEMM, etc.
- We classify parameters as:
    - Numerical (problem size): extrapolation via fitting a univariate piecewise-linear model (e.g., using MARS) to each corresponding factor matrix column (or at least the first one)
    - Architectural: not validated yet, but is naturally more difficult because there are far fewer of them, and the trends are naturally more difficult to predict.
    - Tuning parameters: extrapolation not really relevant here, especially not for categorical (e.g., algorithmic choice) parameters

1. Linear extrapolation (construct a line using the last two elements of each factor matrix). This requires the fewest changes, but also requires knowledge of the largest value in a latent test set. We simply update a final element in each factor matrix column using linear extrapolation of the previous two elements (even if the gap in ranges is huge). Utilizing more dots would not improve the accuracy.

2. fit a MARS model and use that instead of my entire interpolation scheme. This runs into an ablation study mentioned below and may seem more first principles as a cost model that e could try to assess accuracy of. Hopefully it is not as accurate and useful for extrapolation only as an extension

3. Since simply in 1D, simply try to use a scheme in which we use linear regression and use a metric that penalizes for too many variables, so incrementally build up complexity by minimizing R2 (the one that penalizes with too many variables). No cross terms or anything needed. No MARS. Only complication is being piecewise, still search space is quite small in 1D if we limit the number of intervals to like 2-3 (all grid-points gets us back to CPR)


==> improvements.tex <==
# List of possible improvements to the paper:
1. Incorporate more high-dimensional applications
   - SLATE PGEQRF
   - SCALAPACK PGEQRF

